A Girl Has A Name, And It's ... Adversarial Authorship Attribution for Deobfuscation

Recent advances in natural language processing have enabled powerful privacy-invasive authorship attribution. To counter authorship attribution, researchers have proposed a variety of rule-based and learning-based text obfuscation approaches. However, existing authorship obfuscation approaches do not consider the adversarial threat model. Specifically, they are not evaluated against adversarially trained authorship attributors that are aware of potential obfuscation. To fill this gap, we investigate the problem of adversarial authorship attribution for deobfuscation. We show that adversarially trained authorship attributors are able to degrade the effectiveness of existing obfuscators from 20-30% to 5-10%. We also evaluate the effectiveness of adversarial training when the attributor makes incorrect assumptions about whether and which obfuscator was used. While there is a a clear degradation in attribution accuracy, it is noteworthy that this degradation is still at or above the attribution accuracy of the attributor that is not adversarially trained at all. Our results underline the need for stronger obfuscation approaches that are resistant to deobfuscation

==> docs/graveyard.tex <==
\subsection{Authorship Attribution}

    Authorship attribution involves identifying the correct author of a document from a range of possible authors.
    %
    It has been a long-standing topic, and researchers have developed a wide range of solutions to the problem. 
    
    Earlier researchers focused more on analysis based on writing style features.  
    %
    Mosteller and Wallace \cite{mosteller1963inference} used the distribution of word counts and basic Bayesian methods to discriminate between 12 disputed federalist papers. 
    %
    Zheng et al. \cite{zheng2006framework} also used stylometric features, which includes four types of writing-style features: lexical, syntactic, structural, and content-specific features. 
    %
    It was shown that all four types of features can contribute to discriminating the original author from online texts. 
    %
    Clark and Hannon \cite{clark2007algorithm} approached from a different angle and showed that authors have their distinct choices of synonyms, which is helpful in identifying the author. 
    
    %
    More recent researchers have combined machine learning methods and deep learning methods with stylometric features to achieve stronger results. 
    %
    Building on previous works, Abbasi and Chen \cite{abbasi2008writeprints} introduced a comprehensive set of stylometric features for authorship attribution, including lexical, syntactic, structural, content-specific, and idiosyncratic attributes. 
    %
    The rich features set, known as “Writeprints”, was used with support vector machine (SVM) and can support up to 100 different authors. 
    %
    Although Writeprints features achieve high performance, they are computationally expensive.
    %
    Hence, “Writeprints-Static” \cite{brennan2012adversarial} was proposed to reduce the computational load but achieve comparable performance with previous work.

    %
    Recent research have shown an advantage of applying deep learning architectures to the attribution problem since finetuning from pretrained models do not require predefined features sets.
    %
    Ruder et al. \cite{ruder2016character} showed in their 2016 work that CNN outperforms most of the other feature-set based algorithms. 
    %
    Furthermore, Howard and Ruder\cite{howard2018universal} proposed in their 2018 paper a new CV-like transfer learning method, Universal Language Model Fine-tuning (ULMFiT), which outperformed the other state-of-the-art methods and proved the effectiveness of deep learning methods. 

    In our research, we took advantage of the previously established features set “Writeprints-Static” \cite{brennan2012adversarial} with the combination of Random Forest to perform authorship attribution.  Although our research uses similar machine learning architecture as prior work, our work incorporates adversarial training which no prior work in this area has done. 

    
\subsection{Authorship Obfuscation}
    
    Due to the demand for better online privacy and defense from authorship attributors, many authorship obfuscation methods have been proposed by researchers to hide the identity of the original author while preserving most of the semantics of the original text. 
    %
    Earlier works proposed methods that can circumvent the detection of stylometric features both manually and automatically. 
     
    \textbf{Manual.} Rao and Rohatgi \cite{rao2000can} were one of the first ones to suggest round-trip machine translation, where the document is translated from English to another language before going back to English, in document obfuscation. 
    %
    Brennan et al \cite{brennan2012adversarial} mentioned imitating the writing style of another specific user manually, obfuscating their writing style consciously when writing, as well as performing automated multi-stepped round-trip machine translation, which involves more than two languages in the process. 
    %
    Manual obfuscations are not scalable due to the limited instructions for other users, while machine translations quite often break the semantic of the original document. Thus more automated methods have been proposed to address these problems.
    
    %
    \textbf{Semi-Automated.} Improving from the previous scalability issue, Anonymouth by McDonald et al \cite{mcdonald2012use,mcdonald2013anonymouth} captured a set of features that are distinct to an author, then suggested possible alternatives to avoid them. 
    %
    Unfortunately, there are still manual obfuscations involved, so the performance would be affected depending on the understanding of the user.
    
    \textbf{Automated.}
    Karadzhov et al. \cite{karadzhov2017case} focused on rule-based obfuscation where it replaces the words that would make the document deviate from the average features, and Castro et al.
    \cite{castro2017author} used another obfuscation approach that simplified the sentence by rules such as removing the words in parenthesis. 
    %
    In addition to rule-based approaches, Mahmood et al. \cite{mahmood2019girl} proposed a model-based approach that uses genetic algorithm to search for words to change so that it has the largest effect to obfuscation.
    %
    Building on top of that, Gröndahl and Asokan proposed ParChoice \cite{grondahl2020effective}.
    %
    It uses the "combinatorial paraphrasing" style transfer technique together with CNN, LSTM on sentence-level paraphrase selection, and with the same genetic algorithm as Mutant-X on document-level data. 
    %
    It is also worth noting that the authors mention the that most of the style transfer techniques are vulnerable to adversarial training.
    %
    Emmery et al. focused on the setting of obfuscation.
    They emphasized an application that fits realistic condition, where the author does not have access to the target architecture and target domain of document\cite{emmery2021adversarial}.  
    
    Although we focus on Mutant-X \cite{mahmood2019girl} and DS-PAN17 \cite{castro2017author} specifically in our research, the other obfuscation methods are as vulnerable to adversarial training which is reinforced in Grondahl \cite{grondahl2020effective} research.
    
    
    
\subsection{Authorship Deobfuscation}

    Authorship deobfuscation involves finding the original author of an obfuscated text. 
    %
    For our purposes, authorship deobfuscation is a reverse engineering approach against obfuscation methods such that we can minimize the effect of obfuscators that are trying to hind the actual identity of the authors.
    
    There are not any previous papers on authorship deobfuscation. However, there has been work concerning a similar field, code deobfuscation. 
    %
    Code deobfuscation has been an increasingly important topic in the field of deobfuscation.
    %
    Multiple works \cite{udupa2005deobfuscation,  rolles2009unpacking, sharif2009automatic} have talked about deobfuscation of virtualization obfuscator obfuscated code. 
    %
    As mentioned in Udupa et al.’s work about code deobfuscation \cite{udupa2005deobfuscation}, code deobfuscation is a reverse engineering approach to the obfuscated programs. 
    %
    While code obfuscation is crucial to prevent attackers from destructing the software, code deobfuscation is also needed to identify the hidden malicious content. 

    % Adversarial training section
    In our research, we propose combining adversarial training in authorhip deobfuscation. Though the use of adversarial training in text classification has grown, to the best knowledge our is the first research which uses adversarial training to defend against authorship obfuscation methods.

    Adversarial training was first described in \cite{goodfellow2014explaining}, who suggested injecting perturbation into the training set so that the trained models are more resistant towards adversarial examples, the examples that are slightly away from the correctly classified examples. 
    %
    It was also suggested that neural networks are vulnerable to these small changes in input. 
    %
    Ever since then, adversarial training has seen increased attention and has been employed in a variety of areas. 
    
    %
    Though adversarial training initially had the strongest use in the domain of image classification, its common use in image classification has helped adversarial training gradually move into text classification as well. 
    %
    Miyato et al. introduced adversarial and virtual adversarial training to texts domain by adding pertubations in word embeddings \cite{miyato2016adversarial}.  
    %
    Dong et al. \cite{ dong2020leveraging} extends the area further by applying semi-supervised adversarial training to cross-lingual text classification. 
    %
    Using adversarial perturbation as attack, Behjati et al. \cite{behjati2019universal} introduce a gradient projection based method that is able to attack a text classifier even in non-targeted circumstances.    


    
